PostCast: Generalizable Postprocessing for Precipitation Nowcasting via Unsupervised Blurriness Modeling

Precipitation nowcasting plays a pivotal role in socioeconomic sectors, especially in severe convective weather warnings. Although notable progress has been achieved by approaches mining the spatiotemporal correlations with deep learning, these methods still suffer severe blurriness as the lead time increases, which hampers accurate predictions for extreme precipitation. To alleviate blurriness, researchers explore generative methods conditioned on blurry predictions. However, the pairs of blurry predictions and corresponding ground truth need to be generated in advance, making the training pipeline cumbersome and limiting the generality of generative models within blur modes that appear in training data. By rethinking the blurriness in precipitation nowcasting as a blur kernel acting on predictions, we propose an unsupervised postprocessing method to eliminate the blurriness without the requirement of training with the pairs of blurry predictions and corresponding ground truth. Specifically, we utilize blurry predictions to guide the generation process of a pre-trained unconditional denoising diffusion probabilistic model (DDPM) to obtain high-fidelity predictions with eliminated blurriness. A zero-shot blur kernel estimation mechanism and an auto-scale denoise guidance strategy are introduced to adapt the unconditional DDPM to any blurriness modes varying from datasets and lead times in precipitation nowcasting. Extensive experiments are conducted on 7 precipitation radar datasets, demonstrating the generality and superiority of our method.

==> Tables/Table1.tex <==

\begin{table*}[t]
\centering
\vskip 0.1in
\caption{The CSI scores of the highest thresholds evaluated by P1 (max pooling 1), P4 (max pooling 4), and P16 (max pooling 16) at time step 12 (about 1 hour lead time).  }
\label{tab:multidataset}
\vskip 0.1in
\begin{center}
% \begin{small}
% \begin{sc}
\resizebox{\textwidth}{!}
{%
\begin{tabular}{c|ccc|ccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{model} & \multicolumn{3}{c|}{SEVIR} & \multicolumn{3}{c|}{HKO7} & \multicolumn{3}{c|}{TAARSARD19} & \multicolumn{3}{c|}{Shanghai} & \multicolumn{3}{c}{SRAD2018} \\
\cline{2-16}
  & P1 & P4 & P16 & P1 & P4 & P16 & P1 & P4 & P16 & P1 & P4 & P16 & P1 & P4 & P16  \\
\midrule
TAU   & 0.008 & 0.014 & 0.028 & 0.051 & 0.064 & 0.104 & 0.010 & 0.017 & 0.021 & 0.023 & 0.029 & 0.040 & 0.031 & 0.028 & 0.025\\
+ours & 0.075 & 0.098 & 0.134 & 0.139 & 0.229 & 0.356 & 0.092 & 0.124 & 0.167 & 0.028 & 0.052 & 0.113 & 0.086 & 0.156 & 0.274 \\
\hline
PredRNN  & 0.013 & 0.014 & 0.017 & 0.006 & 0.008 & 0.018 & 0.008 & 0.010 & 0.012 & 0.009 & 0.012 & 0.020 & 0.043 & 0.044 & 0.051\\
+ours & 0.080 & 0.103 & 0.135  & 0.124 &  0.214 & 0.344 & 0.085 & 0.115 & 0.161 & 0.026 & 0.050 & 0.109 & 0.083 & 0.154 & 0.277\\
\hline
SimVP & 0.015 & 0.016 & 0.024 & 0.042 & 0.049 & 0.067 & 0.000 & 0.000 & 0.002 & 0.025 & 0.030 & 0.060 & 0.057 & 0.049 & 0.047 \\
+ours & 0.098 & 0.114 & 0.140 & 0.147 & 0.237 & 0.362 & 0.093 & 0.124 & 0.169 & 0.030 & 0.054 & 0.115 & 0.096 & 0.172 & 0.302 \\
\hline
EarthFormer & 0.032 & 0.024 & 0.023 & 0.025 & 0.025 & 0.035 & 0.019 & 0.021 & 0.028 & 0.021 & 0.029 & 0.055 & 0.036 & 0.034 & 0.040 \\
+ours & 0.090 & 0.101 & 0.121 & 0.141 & 0.225 & 0.350 & 0.085 & 0.114 & 0.158 & 0.029 & 0.052 & 0.111 & 0.096 & 0.168 & 0.290 \\
\bottomrule
\end{tabular}
}
\end{center}
\label{tab:1}
\end{table*}


==> Tables/Table2_wrap.tex <==
\begin{wraptable}{l}{12cm}
\centering
\vskip 0.1in
\caption{ The CSI scores of the highest thresholds evaluated by P16 (max pooling 16) at different lead times. }
\label{hko7_meteonet-table}
\vskip 0.1in
\begin{center}
% \begin{small}
% \begin{sc}
\begin{tabular}{l|ccc|ccc}
\toprule
\multirow{2}{*}{model} & \multicolumn{3}{c|}{SEVIR} & \multicolumn{3}{c}{HKO7} \\
\cline{2-7}
 & t=1h & t=2h & t=3h & t=1h & t=2h & t=3h \\
\midrule
TAU   & 0.008 & 0.000 & 0.000 &  0.104 & 0.034 & 0.014 \\
+ours & 0.140 & 0.145 & 0.128 & 0.349 & 0.369 & 0.368 \\
\hline
PredRNN  & 0.017 & 0.000 & 0.000 & 0.018 & 0.003 & 0.001 \\
+ours & 0.140 & 0.146 & 0.127 & 0.350 & 0.367 & 0.364 \\
\hline
SimVP  & 0.024 & 0.005 &  0.000 &  0.067 & 0.024 & 0.017 \\
+ours & 0.142 & 0.146 & 0.128 & 0.363 & 0.366 & 0.362 \\
\hline
EarthFormer & 0.023 & 0.002 & 0.000 & 0.035 & 0.014 & 0.005 \\
+ours & 0.140 & 0.131 & 0.115 & 0.347 & 0.366 & 0.367  \\
\bottomrule
\end{tabular}
\end{center}
\label{tab:2}
\end{wraptable}




==> Tables/Table3.tex <==
\begin{table*}[t]
\centering
\vskip 0.1in
\caption{Zero-shot evaluation. The CSI scores are calculated within the highest thresholds at a lead time of 1 hour. P1, P4, and P16 indicate max pooling 1, max pooling 4, and max pooling 16, respectively. }
\label{hko7_meteonet-table}
\vskip 0.1in
\begin{center}
% \begin{small}
% \begin{sc}
% \resizebox{\textwidth}{!}
{%
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{model} & \multicolumn{3}{c|}{SCWDS CAP30} & \multicolumn{3}{c|}{SCWDS CR} & \multicolumn{3}{c}{MeteoNet} \\
\cline{2-10}
 & P1 & P4& P16 &  P1 & P4& P16 & P1 & P4& P16 \\
\midrule
TAU   & 0.038 & 0.042 & 0.064 & 0.082 & 0.075 & 0.082 & 0.001 & 0.003 & 0.016 \\
+CasCast & 0.068 & 0.115 & 0.254 & 0.118 & 0.180 & 0.336 & 0.029 & 0.067 & 0.128 \\
+DiffCast & 0.022 & 0.047 & 0.147 & 0.040 & 0.081 & 0.222 & 0.001 &  0.004 & 0.026 \\
+ours & 0.205 & 0.257 & 0.347 & 0.329 & 0.412 & 0.509 & 0.046 & 0.078 & 0.135 \\
\hline
PredRNN  & 0.003 & 0.004 & 0.008 & 0.040 & 0.043 & 0.066 & 0.000 & 0.000 & 0.002 \\
+CasCast & 0.052 & 0.086 & 0.189 & 0.086 & 0.139 & 0.283 & 0.021 & 0.046 & 0.135 \\
+DiffCast & 0.027 & 0.049 & 0.139 & 0.069 & 0.108 & 0.246 & 0.012 & 0.028 & 0.092 \\
+ours & 0.205 &  0.257 & 0.352 & 0.330 & 0.413 & 0.510 & 0.045 & 0.077 & 0.135 \\
\hline
SimVP    & 0.025 & 0.026 & 0.035 & 0.056 & 0.046 & 0.041 & 0.000 & 0.000 & 0.002 \\
+CasCast &  0.071 & 0.119 & 0.251 & 0.109 & 0.173 & 0.326 & 0.022 & 0.053 & 0.149 \\
+DiffCast & 0.031 & 0.054 & 0.155 & 0.069 & 0.102& 0.214 & 0.063 & 0.099 & 0.209 \\
+ours &0.201 & 0.254 & 0.348 & 0.333 & 0.414 & 0.510 & 0.097 & 0.153 & 0.249 \\
\hline
EarthFormer & 0.021 & 0.024 & 0.036 & 0.072 & 0.065 & 0.063 & 0.000 & 0.003 & 0.008 \\
+CasCast & 0.066 & 0.111 & 0.240 & 0.110 & 0.169 & 0.314 & 0.024 & 0.059 & 0.159 \\
+DiffCast & 0.046 &  0.078 & 0.191 & 0.100 & 0.143 & 0.280 & 0.012 & 0.034 & 0.118 \\
+ours & 0.191 & 0.238 & 0.332 & 0.323 & 0.397 & 0.489 & 0.092 & 0.144 & 0.235 \\



\bottomrule
\end{tabular}
}
\end{center}
\label{tab:3}
\end{table*}

==> Tables/Table3_SSIM_FID.tex <==
% \begin{table*}[t]
% \centering
% \vskip 0.1in
% \caption{zero-shot to different datasets. }
% \label{hko7_meteonet-table}
% \vskip 0.1in
% \begin{center}
% % \begin{small}
% % \begin{sc}
% \resizebox{\textwidth}{!}
% {%
% \begin{tabular}{l|ccc|ccc|ccc}
% \toprule
% \multirow{2}{*}{model} & \multicolumn{3}{c|}{SCWDS CAP30} & \multicolumn{3}{c|}{SCWDS CR} & \multicolumn{3}{c}{MeteoNet} \\
% \cline{2-10}
%  & P1 & P4& P16 &  P1 & P4& P16 & P1 & P4& P16 \\
% \midrule
% TAU   & 0.038 & 0.042 & 0.064 & 0.082 & 0.075 & 0.082 & 0.001 & 0.003 & 0.016 \\
% +CasCast & & &  & & & & & & \\
% +DiffCast & & &  & & & & & & \\
% +ours & & &  & & & & & & \\
% \hline
% PredRNN  & 0.003 & 0.004 & 0.008 & 0.040 & 0.043 & 0.066 & 0.000 & 0.000 & 0.002 \\
% +CasCast & & &  & & & & & & \\
% +DiffCast & & &  & & & & & & \\
% +ours & & &  & & & & & & \\
% \hline
% SimVP    & 0.025 & 0.026 & 0.035 & 0.056 & 0.046 & 0.041 & 0.000 & 0.000 & 0.002 \\
% +CasCast &  0.055 & 0.090 & 0.208 & 0.076 & 0.116 & 0.250& 0.036 & 0.076 & 0.209 \\
% +DiffCast & 0.024 & 0.044 & 0.129 & 0.047 & 0.071& 0.169 & 0.017 & 0.037 & 0.120 \\
% +ours & & &  & & & & & & \\
% \hline
% EarthFormer & 0.021 & 0.024 & 0.036 & 0.072 & 0.065 & 0.063 & 0.000 & 0.003 & 0.008 \\
% +CasCast & & &  & & & & & & \\
% +DiffCast & & &  & & & & & & \\
% +ours & 0.191 & 0.238 & 0.332 & 0.323 & 0.397 & 0.489 & 0.092 & 0.144 & 0.235 \\



% \bottomrule
% \end{tabular}
% }
% \end{center}
% \label{tab:2}
% \end{table*}

\begin{table*}[t]
\centering
\vskip 0.1in
\caption{Zero-shot evaluation. The CSI scores are calculated within the highest thresholds at a lead time of 1 hour. P1, P4, and P16 indicate max pooling 1, max pooling 4, and max pooling 16, respectively. }
\label{hko7_meteonet-table}
\vskip 0.1in
\begin{center}
% \begin{small}
% \begin{sc}
% \resizebox{\textwidth}{!}
{%
\begin{tabular}{l|ccccc|ccccc|ccccc}
\toprule
\multirow{2}{*}{model} & \multicolumn{5}{c|}{SCWDS CAP30} & \multicolumn{5}{c|}{SCWDS CR} & \multicolumn{5}{c}{MeteoNet} \\
\cline{2-16}
 & SSIM & FID & P1 & P4& P16 & SSIM & FID & P1 & P4& P16 & SSIM & FID & P1 & P4& P16 \\
\midrule
TAU   & & & 0.038 & 0.042 & 0.064 & & & 0.082 & 0.075 & 0.082 & & & 0.001 & 0.003 & 0.016 \\
% +CasCast & 0.068 & 0.115 & 0.254 & 0.118 & 0.180 & 0.336 & 0.029 & 0.067 & 0.128 \\
% +DiffCast & 0.022 & 0.047 & 0.147 & 0.040 & 0.081 & 0.222 & 0.001 &  0.004 & 0.026 \\
% +ours & 0.205 & 0.257 & 0.347 & 0.329 & 0.412 & 0.509 & 0.046 & 0.078 & 0.135 \\
% \hline
% PredRNN  & 0.003 & 0.004 & 0.008 & 0.040 & 0.043 & 0.066 & 0.000 & 0.000 & 0.002 \\
% +CasCast & 0.052 & 0.086 & 0.189 & 0.086 & 0.139 & 0.283 & 0.021 & 0.046 & 0.135 \\
% +DiffCast & 0.027 & 0.049 & 0.139 & 0.069 & 0.108 & 0.246 & 0.012 & 0.028 & 0.092 \\
% +ours & 0.205 &  0.257 & 0.352 & 0.330 & 0.413 & 0.510 & 0.045 & 0.077 & 0.135 \\
% \hline
% SimVP    & 0.025 & 0.026 & 0.035 & 0.056 & 0.046 & 0.041 & 0.000 & 0.000 & 0.002 \\
% +CasCast &  0.071 & 0.119 & 0.251 & 0.109 & 0.173 & 0.326 & 0.022 & 0.053 & 0.149 \\
% +DiffCast & 0.031 & 0.054 & 0.155 & 0.069 & 0.102& 0.214 & 0.063 & 0.099 & 0.209 \\
% +ours &0.201 & 0.254 & 0.348 & 0.333 & 0.414 & 0.510 & 0.097 & 0.153 & 0.249 \\
% \hline
% EarthFormer & 0.021 & 0.024 & 0.036 & 0.072 & 0.065 & 0.063 & 0.000 & 0.003 & 0.008 \\
% +CasCast & 0.066 & 0.111 & 0.240 & 0.110 & 0.169 & 0.314 & 0.024 & 0.059 & 0.159 \\
% +DiffCast & 0.046 &  0.078 & 0.191 & 0.100 & 0.143 & 0.280 & 0.012 & 0.034 & 0.118 \\
% +ours & 0.191 & 0.238 & 0.332 & 0.323 & 0.397 & 0.489 & 0.092 & 0.144 & 0.235 \\



\bottomrule
\end{tabular}
}
\end{center}
\label{tab:3}
\end{table*}

==> Tables/table2.tex <==
\begin{table}[t]
\centering
\vskip 0.1in
\caption{ The CSI scores of the highest thresholds evaluated by P16 (max pooling 16) at different lead times. }
\label{hko7_meteonet-table}
\vskip 0.1in
\begin{center}
% \begin{small}
% \begin{sc}
\begin{tabular}{l|ccc|ccc}
\toprule
\multirow{2}{*}{model} & \multicolumn{3}{c|}{SEVIR} & \multicolumn{3}{c}{HKO7} \\
\cline{2-7}
 & t=1h & t=2h & t=3h & t=1h & t=2h & t=3h \\
\midrule
TAU   & 0.008 & 0.000 & 0.000 &  0.104 & 0.034 & 0.014 \\
+ours & 0.140 & 0.145 & 0.128 & 0.349 & 0.369 & 0.368 \\
\hline
PredRNN  & 0.017 & 0.000 & 0.000 & 0.018 & 0.003 & 0.001 \\
+ours & 0.140 & 0.146 & 0.127 & 0.350 & 0.367 & 0.364 \\
\hline
SimVP  & 0.024 & 0.005 &  0.000 &  0.067 & 0.024 & 0.017 \\
+ours & 0.142 & 0.146 & 0.128 & 0.363 & 0.366 & 0.362 \\
\hline
EarthFormer & 0.023 & 0.002 & 0.000 & 0.035 & 0.014 & 0.005 \\
+ours & 0.140 & 0.131 & 0.115 & 0.347 & 0.366 & 0.367  \\
\bottomrule
\end{tabular}
\end{center}
\label{tab:2}
\end{table}


==> Tables/table_3_2_.tex <==
\begin{table}[t]\small
  \centering
  \caption{Zero-shot evaluation. The CSI scores are calculated within the highest thresholds at a lead time of 1 hour. P1, P4, and P16 indicate max pooling 1, max pooling 4, and max pooling 16, respectively. }
  \label{tab:3(2)}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{c|c c c |c c c | c c c }
    \toprule[1pt]
     \multirow{2}{*}{Model}&\multicolumn{3}{c|}{SCWDS CAP30}&\multicolumn{3}{c|}{SCWDS CR}&\multicolumn{3}{c}{MeteoNet}\\
     \cmidrule(lr){2-10}
     
    &P1&P4&P16&P1&P4&P16&P1&P4&P16\\
    \midrule
TAU   & 0.038 & 0.042 & 0.064 & 0.082 & 0.075 & 0.082 & 0.001 & 0.003 & 0.016 \\
+CasCast & 0.068 & 0.115 & 0.254 & 0.118 & 0.180 & 0.336 & 0.029 & 0.067 & 0.128 \\
+DiffCast & 0.022 & 0.047 & 0.147 & 0.040 & 0.081 & 0.222 & 0.001 &  0.004 & 0.026 \\
+ours & 0.205 & 0.257 & 0.347 & 0.329 & 0.412 & 0.509 & 0.046 & 0.078 & 0.135 \\
\midrule
PredRNN  & 0.003 & 0.004 & 0.008 & 0.040 & 0.043 & 0.066 & 0.000 & 0.000 & 0.002 \\
+CasCast & 0.052 & 0.086 & 0.189 & 0.086 & 0.139 & 0.283 & 0.021 & 0.046 & 0.135 \\
+DiffCast & 0.027 & 0.049 & 0.139 & 0.069 & 0.108 & 0.246 & 0.012 & 0.028 & 0.092 \\
+ours & 0.205 &  0.257 & 0.352 & 0.330 & 0.413 & 0.510 & 0.045 & 0.077 & 0.135 \\
\midrule
SimVP    & 0.025 & 0.026 & 0.035 & 0.056 & 0.046 & 0.041 & 0.000 & 0.000 & 0.002 \\
+CasCast &  0.071 & 0.119 & 0.251 & 0.109 & 0.173 & 0.326 & 0.022 & 0.053 & 0.149 \\
+DiffCast & 0.031 & 0.054 & 0.155 & 0.069 & 0.102& 0.214 & 0.063 & 0.099 & 0.209 \\
+ours &0.201 & 0.254 & 0.348 & 0.333 & 0.414 & 0.510 & 0.097 & 0.153 & 0.249 \\
\midrule
EarthFormer & 0.021 & 0.024 & 0.036 & 0.072 & 0.065 & 0.063 & 0.000 & 0.003 & 0.008 \\
+CasCast & 0.066 & 0.111 & 0.240 & 0.110 & 0.169 & 0.314 & 0.024 & 0.059 & 0.159 \\
+DiffCast & 0.046 &  0.078 & 0.191 & 0.100 & 0.143 & 0.280 & 0.012 & 0.034 & 0.118 \\
+ours & 0.191 & 0.238 & 0.332 & 0.323 & 0.397 & 0.489 & 0.092 & 0.144 & 0.235 \\
    \bottomrule[1pt]

  \end{tabular}
  }
\end{table}

==> Tables/table_3_3_.tex <==
\begin{table}[t]\small
  \centering
  \caption{Zero-shot evaluation. The CSI scores are calculated within the highest thresholds at a lead time of 1 hour. P1, P4, and P16 indicate max pooling 1, max pooling 4, and max pooling 16, respectively. }
  \label{tab:3}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{c|c c c c c|c c c c c| c c c c c}
    \toprule[1pt]
     \multirow{2}{*}{Model}&\multicolumn{5}{c|}{SCWDS CAP30}&\multicolumn{5}{c|}{SCWDS CR}&\multicolumn{5}{c}{MeteoNet}\\
     \cmidrule(lr){2-16}
     
    &FID&SSIM&P1&P4&P16&FID&SSIM&P1&P4&P16&FID&SSIM&P1&P4&P16\\
    \midrule
TAU   & 0.0 & 0.0 & 0.038 & 0.042 & 0.064 & 0.0 & 0.0 & 0.082 & 0.075 & 0.082 & 0.0 & 0.0 & 0.001 & 0.003 & 0.016 \\
+CasCast & 0.0 & 0.0 & 0.067 & 0.102 & 0.224 & 0.0 & 0.0 & 0.101 & 0.145 & 0.258 & 0.0 & 0.0 & 0.029 & 0.067 & 0.128 \\
+DiffCast & 0.0 & 0.0 & 0.023 & 0.050 &0.166 & 0.0 & 0.0 & 0.051 & 0.101 & 0.245 & 0.0 & 0.0 & 0.006 &  0.015 & 0.063 \\
+ours & 40.88 & 0.2034 & 0.075 & 0.126 & 0.269 & 40.32 & 0.3182 & 0.143 & 0.214 & 0.338 & 38.70 & 0.2171 & 0.024 & 0.059 & 0.182 \\
\midrule
PredRNN  & 0.0 & 0.0 & 0.003 & 0.004 & 0.008 & 0.0 & 0.0 & 0.040 & 0.043 & 0.066 & 0.0 & 0.0 & 0.000 & 0.000 & 0.002 \\
+CasCast & 0.0 & 0.0 & 0.035 & 0.056 & 0.129 & 0.0 & 0.0 & 0.086 & 0.139 & 0.283 & 0.0 & 0.0 & 0.010 & 0.030 & 0.101 \\
+DiffCast & 0.0 & 0.0 & 0.017 & 0.035 & 0.102 & 0.0 & 0.0 & 0.066 & 0.105 & 0.230 & 0.0 & 0.0 & 0.006 & 0.019 & 0.076 \\
+ours & 42.56 & 0.1333 & 0.060 &  0.126 & 0.267 & 40.00 &0.3770  & 0.140 & 0.206 & 0.315 & 39.25 & 0.1508 &  0.022 & 0.050 & 0.148 \\
\midrule
SimVP    & 0.0 & 0.0 & 0.025 & 0.026 & 0.035 & 0.0 & 0.0 & 0.056 & 0.046 & 0.041 & 0.0 & 0.0 & 0.000 & 0.000 & 0.002 \\
+CasCast & 0.0 & 0.0 &  0.069 & 0.111 & 0.226 & 0.0 & 0.0 & 0.098 & 0.134 & 0.242 & 0.0 & 0.0 & 0.030 & 0.053 & 0.149 \\
+DiffCast & 0.0 & 0.0 & 0.024 & 0.044 &0.129 & 0.0 & 0.0 & 0.047 & 0.071 & 0.169 & 0.0 & 0.0 & 0.017 & 0.037 & 0.105 \\
+ours & 41.59 & 0.2652 & 0.085 & 0.136 & 0.255 & 40.92 & 0.2924 & 0.140 & 0.205 &  0.296 & 39.42 & 0.020 & 0.020 & 0.052 & 0.144 \\
\midrule
EarthFormer & 0.0 & 0.0 & 0.021 & 0.024 & 0.036 & 0.0 & 0.0 & 0.072 & 0.065 & 0.063 & 0.0 & 0.0 & 0.000 & 0.003 & 0.008 \\
+CasCast & 0.0 & 0.0 & 0.050 & 0.089 & 0.190 & 0.0 & 0.0 & 0.100 & 0.130 & 0.223 & 0.0 & 0.0 & 0.019 & 0.055 & 0.159 \\
+DiffCast & 0.0 & 0.0 & 0.041 &  0.071 & 0.175 & 0.0 & 0.0 & 0.101 & 0.144 & 0.268 & 0.0 & 0.0 & 0.009 & 0.029 & 0.096 \\
+ours & 41.36 & 
 0.2637 & 0.070 & 0.117 & 0.241 & 40.65 & 0.1875 & 0.141 & 0.211 & 0.326 & 38.58 & 0.2488 & 0.019 & 0.058 & 0.164 \\
    \bottomrule[1pt]

  \end{tabular}
  }
\end{table}
